An LSTM model for Twitter Sentiment Analysis

Sentiment analysis on social media such as Twitter provides organizations and individuals an effective way to monitor public emotions towards them and their competitors. As a result, sentiment analysis has become an important and challenging task. In this work, we have collected seven publicly available and manually annotated twitter sentiment datasets. We create a new training and testing dataset from the collected datasets. We develop an LSTM model to classify sentiment of a tweet and evaluate the model with the new dataset.

==> relatedwork.tex <==
\section{Related work}\label{sec:relatedworkd}

==> tasks.tex <==
\section{Tasks}\label{sec:tasks}
In this work, the tasks can be divided into four parts.
\begin{itemize}
  \item Data preprocessing: Some of the datasets only have tweet ids and sentiment labels. We need to extract tweet text by using the tweet ids and twitter api.
  \item New Dataset construction: We will create the new training dataset by taking $90\%$ of data from each dataset and the remaining $10\%$ will be used to create the new testing set.  
  \item LSTM model implementation: We will use keras with tensorflow to implement the LSTM model. The tweet text needs to be preprocessed before feeding it to the model. The preprocessing steps include word tokenization, replacing hashtag/user mentions/urls/emoticons/punctuations with fixed keywords, removing repeating characters, word embeddings. 
  \item Experimental evaluation: To measure the performance of the LSTM model, we will use accuracy, precision, recall, and F1 score as evaluation metrics.
\end{itemize}
